Distributed Adaptive Backstepping Control for Vehicular Platoons with Mismatched Disturbances Using Vector String Lyapunov Functions

In this paper, we consider the problem of platooning control with mismatched disturbances using the distributed adaptive backstepping method. The main challenges are: (1) maintaining the compositionality and the distributed nature of the controller, and (2) ensuring the robustness of the controller with respect to general types of disturbances. To address these challenges, we first propose a novel notion that we named "Vector String Lyapunov Function", whose existence implies l2 weak string stability. This notion is based on the vector Lyapunov function-based stability analysis, which depends on the input-to-state-stability of a comparison system. Using this notion, we propose an adaptive backstepping controller for the platoon such that the compositionality and the distributed nature of the controller can be ensured while the internal stability and string stability of the closed-loop system are formally guaranteed. Finally, simulation examples are provided to illustrate the effectiveness of the proposed control algorithm. In particular, we provide simulation results comparing our proposed control algorithm with a recently proposed control algorithm from the literature, under two types of information flow topologies and disturbances.

==> oldtexfiles/additional.tex <==
To determine the corresponding partition in the abstraction's space, i.e. \(\mathbf{D}_{zj}z\geq \mathbf{E}_{zj}\), based on the desired partition in concrete system's space, i.e. \(\mathbf{D}_{j}x\geq \mathbf{E}_{j}\), the following lemma is applied:

\begin{lemma} \cite{??,??}
    Given a polytope \(\mathcal{Z}=\{\mathbf{z}\in\mathbb{R}^m|\mathbf{D}_{zj}\mathbf{z}\geq \mathbf{E}_{zj}\}\), \(\mathbf{P}_i\in\mathbb{R}^{n\times m}\), \(\mathbf{\hat{y}}\in\mathbb{R}^n\), and \(\mathcal{X}_j=\{\mathbf{x}\in\mathbb{R}^n|\mathbf{D}_j\mathbf{x}\geq \mathbf{E}_j\}\), \(j=1,...,r\), the condition \(\mathbf{P}_i\mathcal{Z}+\mathbf{\hat{y}}\subseteq\mathcal{X}_j\) is equivalent to
    \begin{equation}
        \mathbf{\Lambda}_k\mathbf{D}_{zj}=\mathbf{D}_{j}\mathbf{Q}_k,\ \sum_{k=1}^{N}\mathbf{\Lambda}_k\mathbf{E}_{zj}\geq \mathbf{E}_j-\mathbf{D}_{j}\mathbf{\hat{y}}
    \end{equation}
    where \(\mathbf{\Lambda}_k\) is some matrix with nonnegative entries, \(\sum_{k=1}^{N} \mathbf{Q}_k=\mathbf{P}_i\).
\end{lemma}
